Time to Reason: Scalable Neurosymbolic Learning for LTLf via Fuzzy Semantics

Neurosymbolic (NeSy) Artificial Intelligence aims to integrate Deep Learning (DL) architectures with symbolic reasoning. While initial NeSy approaches have targeted mainly symbolic reasoning in propositional and first-order logics, recent works have started to address the construction of neurosymbolic frameworks for Temporal Logics, and in particular for LTLf. These approaches have established temporal NeSy as a promising research direction, laying the foundations for learning under temporal constraints. Nonetheless, they leave many questions unanswered. From a theoretical perspective, several differentiable semantics for interpreting LTLf have been proposed but have not yet been formally and systematically defined within a unified framework. Moreover, existing approaches commonly rely on automata to represent temporal knowledge, resulting in limited scalability. Motivated by this research gap, this paper provides the following contributions: (i) formally defining different fuzzy semantics for LTLf, and systematically analysing theoretical properties regarding equivalences and dualities of temporal operators; (ii) showing how these semantics can be directly integrated within a novel NeSy framework, called DiffLTLf, enabling flexible and scalable learning without relying on the usage of automata; and (iii) introducing a novel evaluation protocol of increased complexity of learning tasks w.r.t. existing benchmarks. Our results show that the choice of fuzzy semantics has a significant impact on predictive performance. Moreover, DiffLTLf achieves performance on par with, and sometimes superior to, state-of-the-art probabilistic approaches while substantially improving scalability. Taken together, these results establish direct fuzzy interpretations as a competitive and scalable alternative to existing temporal NeSy frameworks.

==> Sections/conceptualComparison-old.tex <==



\section{State of the Art}
\label{sec:sota}

In this section we review the state of the art in neurosymbolic (NeSy) learning, covering both approaches designed for static, relational domains, that is, domains where knowledge is formalised using propositional or first-order logics,  (Section \ref{sec:sota_static}) and those addressing temporal domains, that is domains where knowledge is formalised using one of the variants of temporal logics,  (Section \ref{sec:sota_temporal}).
For each, we describe how symbolic knowledge is integrated into the learning process, and we discuss their merits and limitations.
This analysis motivates the design choices behind \DiffLTLf, which we introduce in the following sections.


\subsection{Neurosymbolic Integration in Static Domains}
\label{sec:sota_static}
NeSy integration aims to bridge neural learning and logical reasoning. In static domains, the NeSy literature can be broadly classified based on where the symbolic knowledge is injected into the machine learning pipeline \cite{informed_ML}\footnote{In the broader taxonomy of informed machine learning \cite{informed_ML}, our ``loss-based'' and ``model-based'' categories correspond to integrating knowledge into the \emph{Learning Algorithm} and the \emph{Hypothesis Space}, respectively.}.
\todo[inline]{Chiara: non capisco se ``loss-based'' and ``model-based'' sono termini che definiamo noi. Se cosi' e' io userei quelli standard di \emph{Learning Algorithm} and the \emph{Hypothesis Space}. Senno' citerei un paper che gia' introduce questa terminologia. Inoltra la footnote andrebbe messa dopo la prima menzione di loss based e non qui.}

The first category comprises \emph{loss-based} approaches, where logic is strictly used to modify the learning algorithm (e.g., as a regularization term). In these frameworks, the neural network is penalised during training for violating logical constraints, but the symbolic component is discarded at inference time. The second category consists of \emph{model-based} approaches, which restrict the model's hypothesis space by embedding logic directly into the computational architecture, ensuring that logical reasoning persists during inference. The historical roots of this architectural integration can be traced back to KBANN \cite{KBANN}, which explicitly compiled symbolic rules into neural network topologies.

Orthogonally to this architectural divide, NeSy frameworks differ in the mathematical formalism used to evaluate logic. \emph{Probabilistic} approaches leverage probabilistic inference. Within this formalism, Semantic Loss \cite{DBLP:conf/icml/XuZFLB18} acts as a loss-based regularizer, whereas frameworks like DeepProbLog \cite{DBLP:conf/nips/ManhaeveDKDR18} and DeepStochLog \cite{DBLP:conf/aaai/WintersMMR22} act as model-based systems, piping neural outputs into probabilistic inference engines. However, the reliance on Weighted Model Counting (WMC) makes scaling probabilistic methods to complex formulas a significant computational bottleneck.

To overcome these scalability issues, \emph{fuzzy logic} frameworks leverage t-norms to translate discrete connectives into differentiable algebraic operations. %Applying the architectural distinction to this paradigm, 
Within the fuzzy logic paradigm, Logic Tensor Networks (LTN) \cite{ltn} and Semantic-Based Regularization (SBR) \cite{SBR} are popular loss-based fuzzy approaches. Conversely, model-based fuzzy approaches~\cite{KENN,DBLP:journals/ml/DanieleKSH23,Giunchiglia1, Giunchiglia2}, embed differentiable logical operations directly into the structure of neural networks through additional differentiable layers. Notably, these model-based methods are typically hardcoded to a specific t-norm semantics, which limits their flexibility across diverse domain constraints.

Despite the success of these frameworks in combining sub-symbolic and symbolic representations, a fundamental limitation shared by all these NeSy frameworks is the lack of native operators to model temporal dependencies.
\todo[inline]{Secondo me questa non e' una limitazione... e' una scelta di usare una logica invece di un'altra. Infatti eliminerei la frase sopra e anche quelle dopo, semplicemente dicendo come \DiffLTLf si piazza in questa classificazione. Questo permette di accorciare anche la sezione.}

In our work, we overcome these limitations by adopting a semantics-agnostic, model-based fuzzy paradigm for temporal data. 
In this respect, while our use of fuzzy semantics to evaluate logical formulas is shared with frameworks such as LTN, our setting differs.
In LTN the knowledge is a constraint to be satisfied, and the logic is used as a regularization term in the loss. 
In our task, the specification is instead a per-sequence label that may either be satisfied or violated, from which the symbol grounding must be learned.
This makes \DiffLTLf a model-based approach, in which the formula is treated as a differentiable computational layer. \footnote{The \DiffLTLf framework is not limited to this setting, as it can be instantiated in a loss-based fashion, and the theoretical analysis of Section \ref{sec:fuzzyLTL} applies unchanged. We leave such extensions to future work.}
% By treating the formula as a differentiable computational layer, we enable scalable, instance-specific supervision that persists at inference time.


\subsection{Neurosymbolic Integration in Temporal Domains}
\label{sec:sota_temporal}
NeSy learning over temporal domains is a recent and small, but rapidly growing, research effort. In this setting, 
% in which the symbolic knowledge captures temporal dependencies among symbols, 
reasoning must capture temporal dependencies among symbols, expressed in 
such as the order in which events may occur. The works we consider here have in fact being published in the last 3 years. A first important observation is that all the recent efforts focus on a particular variant of Temporal Logics, that is, Linear time Temporal Logics on finite traces (\LTLF). 

Existing frameworks differ along two main dimensions: how the temporal knowledge is integrated into the learning process, and which differentiable semantics is used to interpret the temporal formula. 

Concerning the way in which temporal knowledge is integrated into the learning process, the dominant approach compiles the \LTLF specification into a deterministic finite-state automaton (DFA), which is then evaluated in a differentiable manner over the perception outputs. The two most representative instances of this approach are \FuzzyDFA \cite{DBLP:conf/kr/UmiliCG23} and \NeSyA \cite{DBLP:conf/ijcai/ManginasPR25}. In these frameworks, at each timestep, a neural perception module produces soft truth values for the atomic propositions, which are used to evaluate the automaton's transition guards.
The guard values then update the truth values associated with each automaton state, recursively from the first to the last instant of the sequence.
%The two most representative instances of this paradigm, \FuzzyDFA \cite{DBLP:conf/kr/UmiliCG23} and \NeSyA \cite{DBLP:conf/ijcai/ManginasPR25}, differ along the second dimension, namely in the semantics they adopt.
The explicit construction of a finite-state automaton from the \LTLF formula originates two distinct limitations:
% Generally, automata-based approaches suffer from two limitations.
First, the automaton must be built before training, and its size is, in the worst case, double-exponential in the size of the \LTLF formula~\cite{DBLP:conf/ijcai/GiacomoV13}.
The second is incurred during training, when the automaton is evaluated. The state valuation is computed recurrently over the sequence, each timestep depending on the previous one, so the evaluation is inherently sequential, preventing parallelisation over time. 
To overcome these limitations, \TILR \cite{DBLP:conf/nesy/AndreoniBDGMR25} operates directly on the logical structure of the formula, foregoing the need for an intermediate DFA-based representation.
In particular, \TILR proposes a differentiable framework in which \LTLF formulas are evaluated through fuzzy semantics without compiling them into an intermediate automaton. This allows the model to compute a degree of satisfaction directly from the neural outputs, while still enabling gradient-based optimization. 

To overcome the two limitations written above we base our proposal \DiffLTLf on this latter approach of evaluating directly \LTLF formulas trough a differentiable semantics without compiling them into an intermediate automaton.

Concerning the differentiable semantics is used to interpret the temporal formula, we can observe an heterogeneous situation. 
\FuzzyDFA and \TILR adopt a fuzzy semantics, while \NeSyA relies on probabilistic reasoning. More in detail, \FuzzyDFA
adopts a fuzzy interpretation of the automaton, and exploits the Product semantics for the fuzzy connectives.\footnote{The same mechanism has been adapted to non-Markovian reinforcement learning \cite{DBLP:conf/nesy/UmiliABC23} and to suffix prediction under \LTLF constraints \cite{DBLP:conf/pmai/UmiliLP24}.} The Product semantics is justified as inherited from Logic Tensor Networks, the NeSy framework that is at the basis of \FuzzyDFA. The fuzzy interpretation of te automaton works as follows: first, the perception module assigns a fuzzy truth value to each atomic proposition at every timestep. Then, each transition guard is evaluated according to fuzzy semantics, and the vector of fuzzy truth values over the automaton states is updated recursively. After the last image, the degree of satisfaction of the formula is obtained by aggregating the fuzzy values of the accepting states.
%The authors of \FuzzyDFA choose to inherit from LTN \cite{ltn} the Product semantics for the fuzzy connectives. 
Instead, \TILR is tied to the G\"{o}del fuzzy semantics. This choice if justified in terms of the theoretical investigation provided in \citet{DonadelloFIMM25}. \todo{Chiara: qui metterei almeno una righina per spiegare il ruolo della semantica fuzzy}
Finally, \NeSyA replaces fuzzy semantics with probabilistic reasoning.
In this approach, the \LTLF formula is compiled into a symbolic finite-state automaton (SFA), where transition guards are represented as logical formulas over atomic propositions. These formulas are further compiled into tractable arithmetic circuits, enabling efficient weighted model counting (WMC). At each timestep, the neural outputs define a probability distribution over truth assignments of atomic propositions, which is used to compute the probability that each transition guard is satisfied. These probabilities determine the transition matrix of the automaton, and the state distribution is updated by multiplication with this matrix at each timestep.
% through standard probabilistic propagation.
The probabilistic semantics is exact and avoids the approximation introduced by fuzzy evaluation. It comes, however, at a computational cost, as weighted model counting must be carried out for every transition at every timestep. 

While the choice of fuzzy or probabilistic semantics for NeSy frameworks may depend upon the task to be solved, and recent studies highlight a trade off between performance vs scalability when choosing among fuzzy logics vs probabilistic logics~\cite{DBLP:conf/nips/MaeneR23}, it is easy to observe that state of the art formalisms lack an in depth theoretical and practical investigation of the impact that this choice has, both in terms of the relationship between the differentiable semantics and the classical one, and in terms of performances. This is a crucial aspect, specially for formalisms based on fuzzy logics, as prior work on propositional logics shows that the choice of fuzzy semantics can significantly affect performance within NeSy frameworks~\cite{DBLP:journals/ai/KriekenAH22}. 

The theoretical investigation proposed in Section \ref{sec:fuzzyLTL} aims at filling the theoretical gap, by providing an investigation of different fuzzy semantics for \LTLF. This investigation is independent of our framework and can be exploited by future efforts in defining temporal NeSy frameworks. Building from this investigation we define \DiffLTLf for different fuzzy semantics. The Evaluation section (Section~\ref{sec:evaluation}) aims instead at filling the practical gap, by investigating the impact that the different fuzzy and probabilistic semantics on performance and scalability. 

It is worth noting that, despite their architectural differences, the methods above are evaluated on a common learning setting, namely distant supervision over temporal data, as introduced in Section~\ref{sec:task_overview}, where supervision is provided only at the sequence level. Nonetheless, all the methods above are evaluated on specifications of low complexity, short sequences, and few propositions over a single perceptual stream, which leaves the scalability of the different approaches under-analysed. 


A recent benchmark related to this setting is \LTLZinc \cite{ltlzincIJCAI}, which targets sequence classification under temporal specifications, but  
% presents several limitations as a general evaluation protocol for temporal NeSy approaches.
is not fully suited to isolating and comparing temporal NeSy methods under purely distant supervision.
First, its specifications interleave temporal operators with relational constraints, so that the contribution of the temporal reasoning component is not isolated.
Second, it introduces intermediate supervision signals at several levels of the pipeline, together with a supervised pre-training of the perception module.
While this facilitates training, it makes the benchmark less suitable for assessing how methods perform when only distant supervision is available.
Third, it relies on the supervision on the next state in the finite-state machine. This makes it applicable only to automata-based methods, excluding approaches that evaluate the temporal specification directly.
These limitations motivate the evaluation protocol we introduce (Section \ref{sec:evaluation}), which relies only on the sequence-level label and applies to both automata-based and automata-free methods. Moreover, our evaluation setting disentangles two distinct sources of difficulty by varying separately the size of the temporal specification and the length of the input sequences.



 construction of a finite-state automaton from the \LTLF formula originates two distinct limitations:


\FuzzyDFA \cite{DBLP:conf/kr/UmiliCG23} adopts a fuzzy interpretation of the automaton.\footnote{The same mechanism has been adapted to non-Markovian reinforcement learning \cite{DBLP:conf/nesy/UmiliABC23} and to suffix prediction under \LTLF constraints \cite{DBLP:conf/pmai/UmiliLP24}.}
The perception module assigns a fuzzy truth value to each atomic proposition at every timestep.
Each transition guard is evaluated according to fuzzy semantics, and the vector of fuzzy truth values over the automaton states is updated recursively.
After the last image, the degree of satisfaction of the formula is obtained by aggregating the fuzzy values of the accepting states.
The fuzzy connectives are instantiated with the Product semantics. While this choice is inherited from LTN \cite{ltn}, it represents a first limitation as the properties of the resulting temporal semantics are not investigated.
A second limitation concerns the experimental evaluation, restricted to specifications of low complexity, short sequences, and few propositions over a single perceptual stream, which leaves the scalability of the approach under-analysed. 
%Our work directly addresses this limitation by studying and comparing different fuzzy semantics for temporal logic (Section \ref{sec:fuzzyLTL}).
\NeSyA \cite{DBLP:conf/ijcai/ManginasPR25}, instead replaces fuzzy semantics with probabilistic reasoning.
In this approach, the \LTLF formula is compiled into a symbolic finite-state automaton (SFA), where transition guards are represented as logical formulas over atomic propositions. These formulas are further compiled into tractable arithmetic circuits, enabling efficient weighted model counting (WMC). At each timestep, the neural outputs define a probability distribution over truth assignments of atomic propositions, which is used to compute the probability that each transition guard is satisfied. These probabilities determine the transition matrix of the automaton, and the state distribution is updated by multiplication with this matrix at each timestep.
% through standard probabilistic propagation.
The probabilistic semantics is exact and avoids the approximation introduced by fuzzy evaluation. It comes, however, at a computational cost, as WMC must be carried out for every transition at every timestep. 
%Our experiments (Section \ref{sec:results}) show that this makes \NeSyA the most computationally demanding of the compared methods, with a cost that grows rapidly as formula complexity and sequence length increase.
A further limitation lies in the evaluation, which uses few propositions and short sequences. Moreover, although the perception module performs symbol grounding, its accuracy is never measured, as only sequence-level classification is reported. As a consequence, the quality of the symbol grounding is left unaddressed.


This motivates a different line of work, which avoids the automaton altogether and evaluates the temporal specification directly on the perception outputs.

A first step in this direction is \TILR \cite{DBLP:conf/nesy/AndreoniBDGMR25}, which operates directly on the logical structure of the formula, foregoing the need for an intermediate DFA-based representation.
In particular, \TILR proposes a differentiable framework in which \LTLF formulas are evaluated through fuzzy semantics without compiling them into an intermediate automaton. This allows the model to compute a degree of satisfaction directly from the neural outputs, while still enabling gradient-based optimization. 
\TILR, however, is tied to a single fuzzy semantics, namely Gödel. While this fuzzy temporal semantics has theoretical foundations \cite{DonadelloFIMM25}, restricting the framework to one semantics is a limitation. As our experiments show (Section \ref{sec:results}), and as already observed in the non-temporal setting~\cite{DBLP:journals/ai/KriekenAH22}, the choice of fuzzy semantics significantly affects performance.
Our work addresses this limitation by formalising and comparing three fuzzy semantics for temporal logic (Section \ref{sec:fuzzyLTL}).
A second limitation, shared with the methods above, concerns the experimental evaluation: although broader than that of \FuzzyDFA, it remains limited in formula complexity, number of propositions, and sequence length.

It is worth noting that, despite their architectural differences, the methods above are evaluated on a common learning setting, namely distant supervision over temporal data, as introduced in Section~\ref{sec:task_overview}, where supervision is provided only at the sequence level.
A recent benchmark related to this setting is \LTLZinc \cite{ltlzincIJCAI}, which targets sequence classification under temporal specifications, but  
% presents several limitations as a general evaluation protocol for temporal NeSy approaches.
is not fully suited to isolating and comparing temporal NeSy methods under purely distant supervision.
First, its specifications interleave temporal operators with relational constraints, so that the contribution of the temporal reasoning component is not isolated.
Second, it introduces intermediate supervision signals at several levels of the pipeline, together with a supervised pre-training of the perception module.
While this facilitates training, it makes the benchmark less suitable for assessing how methods perform when only distant supervision is available.
Third, it relies on the supervision on the next state in the finite-state machine. This makes it applicable only to automata-based methods, excluding approaches that evaluate the temporal specification directly.
These limitations motivate the evaluation protocol we introduce (Section \ref{sec:evaluation}), which relies only on the sequence-level label and applies to both automata-based and automata-free methods. Moreover, our evaluation setting disentangles two distinct sources of difficulty by varying separately the size of the temporal specification and the length of the input sequences.
















% R: da qui c'è la vecchia sezione
\endinput

\section{Nesy Frameworks for Temporal Logic}
\label{sec:conceptual}
%% Labels are used to cross-reference an item using \ref command.
In this section, we describe some of the existing frameworks focusing on neurosymbolic (NeSy) learning over temporal domains. Although most efforts have focused on NeSy over static, relational domains~\cite{DBLP:series/faia/BesoldGBBDHKLLPPPZ21}, recent efforts have started proposing solutions for NeSy learning over temporal domains, dealing with different types of formalisms, architectures, and evaluation protocols.

The most popular choice of temporal NeSy approaches is based on the representation of \LTLF formulae into deterministic finite automata (DFAs), which provide a way of evaluating temporal specifications over sequences~\cite{DBLP:conf/kr/UmiliCG23,DBLP:conf/ijcai/ManginasPR25}. Given an input sequence, a neural perception module produces, at each timestep, a vector of soft truth values corresponding to the atomic propositions appearing in the formula. These values are then used to evaluate the transition guards of the automaton. 
In order to provide learning signals for these perception modules, different ways of interpreting the truth values of the knowledge have been explored; either through the use of fuzzy logics~\cite{DBLP:conf/kr/UmiliCG23} or probabilistic interpretations of the truth values~\cite{DBLP:conf/ijcai/ManginasPR25}. 



The former approach, instantiated in \FuzzyDFA~\cite{DBLP:conf/kr/UmiliCG23}, treat each transition guard as a fuzzy propositional formula. The automaton is executed over the sequence by maintaining a %distribution over states
vector of fuzzy truth values over states, which is updated recursively at each timestep. Concretely, the current state truth values are combined with the fuzzy evaluation of transition conditions to produce the %next state distribution
next state values, typically via a differentiable relaxation of logical conjunctions and disjunctions. The final degree of satisfaction of the \LTLF formula is obtained from the %probability mass assigned to accepting states 
fuzzy truth values assigned to accepting states 
after processing the entire sequence. This value is then used to create the supervision signal, enabling gradient-based optimization in weakly supervised settings. %\todo[inline]{Ale: non direi che e' un supervision signal. Forse e' meglio dire che viene usato per creare il supervision signal}
% While this approach enables end-to-end differentiability, the supervision signal is obtained only after propagating the truth values %a distribution\todo{Ale: se parliamo di fuzzy logic non e' corretto parlare di distribuzione}
% over automaton states across the entire sequence. As a result, the contribution of early timesteps is progressively diluted, making it harder to learn long-range temporal dependencies. In addition, the need to maintain and update the fuzzy truth values %a full state distribution\todo{Ale: di nuovo, non userei il termine distribution}
% at each step introduces a computational cost that scales with the size of the automaton.

An alternative formulation is provided by \NeSyA, which replaces fuzzy semantics with probabilistic reasoning. In this approach, the \LTLF formula is compiled into a symbolic finite automaton (SFA), where transition guards are represented as logical formulas over atomic propositions. These formulas are further compiled into tractable arithmetic circuits, enabling efficient weighted model counting (WMC)~\cite{DBLP:conf/ijcai/ManginasPR25}. At each timestep, the neural outputs define a probability distribution over truth assignments of atomic propositions, which is used to compute the probability that each transition guard is satisfied. These probabilities determine the transition matrix of the automaton, and the state distribution is updated through standard probabilistic propagation. While this formulation provides a principled way to model uncertainty, it introduces additional computational overhead due to the construction and evaluation of probabilistic circuits, which may become prohibitive for complex temporal formulas or large sets of proposition.

The general issue with DFA-based approaches is two-fold: the translation of an \LTLF formula into a DFA or SFA can incur a double-exponential blow-up in the number of states~\cite{DBLP:conf/ijcai/GiacomoV13}, which directly impacts both memory usage and computational cost. Moreover, this may have cascading consequences when dealing with complex temporal specifications or large formula sets within the training procedure, as the DFA has to be repeatedly traversed during training, which may incur high overall computational costs.%\todo[inline]{Ale: curiosita': cosa intendi con "for each separate input"? Immagino che ogni input sia fatto in parallelo: per ogni transizione, si calcola sempre un vettore di probabilita' sugli stati, no? Quindi le dimensioni dei vettori dovrebbe sempre essere lo stesso, e anche le operazioni fatte, dunque dovrebbe essere parallelizzabile. Se cosi' fosse, non specificherei che e' per ogni singolo input}


A recent solution to address this limitation was proposed in the literature, namely \TILR~\cite{DBLP:conf/nesy/AndreoniBDGMR25}, by directly operating on the logical structure of the formula, foregoing the need for an intermediate DFA-based representation. In particular, \TILR proposes a differentiable framework in which \LTLF formulas are evaluated through fuzzy semantics without compiling them into an intermediate automaton. This allows the model to compute a degree of satisfaction directly from the neural outputs, while still enabling gradient-based optimization. However, this approach is tied to a specific choice of fuzzy semantics, which may limit its flexibility. This is particularly relevant as prior work has shown that the choice of fuzzy semantics can significantly affect performance in NeSy systems~\cite{DBLP:journals/ai/KriekenAH22}.

%\todo[inline]{Ale: non sono convinto che sia corretto mettere questa parte qui, visto che si tratta piu' che altro di un banchmark. In generale, sembra un po' scollegato il discorso, secondo me non fila perfettamente. Forse vale la pena una sezione a parte? In ogni caso, andrei direttamente al paragrafo dopo (It is worth noting that, ...), e se lasciamo \LTLZinc in questa sezione, magari metterei l'introduzione ad esso direttamente in quella sezione}
%\todo[inline]{Andrei: Ci sta, comunque con Ricc ci era venuto il dubbio che alcune parti potrebbero essere riportate meglio nella sezione di rel work. Forse questo proporio andrebbe spostata li'. Al momento, ho spostato una frase sotto per introdurre ltlzinc visto che ne parliamo, il resto l'ho spostato in related}
%Finally, an important step toward the standardization of evaluation in this area is represented by the introduction of the \LTLZinc benchmark~\cite{ltlzincIJCAI}. \LTLZinc provides a unified benchmarking framework for NeSy temporal reasoning, focusing on sequence classification tasks with relational and temporal constraints. It defines a modular pipeline that enables systematic comparison between approaches such as \FuzzyDFA and \NeSyA, while highlighting key challenges including scalability and robustness to perception errors.
%However, the framework is inherently tied to the automata-based paradigm, as it relies on DFA constructs to generate supervision signals. As a result, it primarily supports DFA-based methods, limiting its ability to fairly evaluate approaches that avoid explicit automaton representations. 


It is worth noting that, despite their architectural differences, all the aforementioned approaches are designed for a common learning setting, namely distant supervision over temporal data, as introduced in Section~\ref{sec:task_overview}. In this setting, supervision is provided only at the sequence level, and the learning signal must be propagated through the temporal reasoning component.
A partial exception is represented by the \LTLZinc benchmark~\cite{ltlzincIJCAI}, focusing on sequence classification tasks with relational and temporal constraint. Differently from distant supervision, in this benchmark, additional intermediate supervision signals are introduced within the pipeline. While this facilitates the training process,
it introduces an additional limitation in that the framework requires multiple levels of supervision in order to actually learn the symbol grounding task, relying for example on the relational constraint satisfaction, and the supervision on the next state in the finite-state machine~\cite{ltlzincIJCAI}, making it inherently limited to the automata-based paradigm.
We believe that this setting deviates from purely distant supervision, making it less suitable to properly assess how these methods perform when only distant supervision is available.
%\begin{enumerate}
%    \item \NeSyA\cite{DBLP:conf/ijcai/ManginasPR25}
%    \item \FuzzyDFA\cite{DBLP:conf/kr/UmiliCG23}
%    \item DeepDfa\cite{DBLP:conf/ecai/UmiliC24} ?
%    \item \LTLZinc\cite{ltlzincIJCAI}
%    \item \TILR\cite{DBLP:conf/nesy/AndreoniBDGMR25} ?
%\end{enumerate}

==> Sections/drawings-old.tex <==


% \InlineNode[options]{name}{text}
%\NewDocumentCommand{\inlinenode}{O{} m m}{%
%  \subnode[inner sep=0pt,outer sep=0pt,#1]{#2}{#3}%
%\subnode[fill=cyan]{c}{ccccc}
%}

\newcommand{\bgcell}[2]{
|[fill=#2]|#1
}

 \newcommand{\fuzzyeval}[3]{\bgcell{#1}{#3!\fpeval{100*#2}}}

\newcommand{\fuzzyval}[1]{
\fuzzyeval{#1}{#1}{LimeGreen}
}

\newcommand{\fuzzya}[1]{
\fuzzyeval{#1}{1}{white}
}

\newcommand{\fuzzyg}[2]{
\fuzzyeval{#1}{#2}{LimeGreen}
}
\newcommand{\fuzzyp}[2]{
\fuzzyeval{#1}{#2}{LimeGreen}
}
\newcommand{\fuzzyl}[2]{
\fuzzyeval{#1}{#2}{LimeGreen}
}

% \newcommand{\formulabox}[2]{
% \colorbox{#2}{\ensuremath{#1}}
% }

\newcommand{\formulabox}[3]{
%\inlinenode[fill=#3]{#1}{\ensuremath{#2}}
\subnode[inner sep=0pt,outer sep=0pt]
    {#1}
    {
        \colorbox{#3}{\ensuremath{#2}}
    }
}



\newcommand{\uformula}{
\ensuremath{a \U b}
}

\newcommand{\nuformula}{
\ensuremath{\X(\uformula)}
}

\newcommand{\aformula}{
\ensuremath{a \land \nuformula}
}

\newcommand{\nucolorzero}{Goldenrod}
\newcommand{\nucolorone}{Dandelion}
\newcommand{\nucolortwo}{BurntOrange}

\newcommand{\acolorzero}{SpringGreen}
\newcommand{\acolorone}{LimeGreen}
\newcommand{\acolortwo}{JungleGreen}

\newcommand{\ucolorzero}{Lavender}
\newcommand{\ucolorone}{Orchid}
\newcommand{\ucolortwo}{Plum}

\newcommand{\atomcolor}{gray!50}


% \tikzset{
%   every matrix/.append style={
%     every cell/.style 2 args={
%       /utils/exec={
%         \ifnum##2>1\relax
%           \tikzset{nodes={text width = 1.5em}}
%         \fi
%       }
%     }
%   }
% }

\tikzstyle{table} = [
    matrix of nodes,
    ampersand replacement=\&,
    row sep=-\pgflinewidth,
    column sep=.5em,
    nodes={
      rectangle,
      draw=black,
      align=center,
      text centered,
      font=\footnotesize\ttfamily
    },
    text height=1em,
    text depth=0.5em,
    %m height=1.5ex,
    nodes in empty cells,
    % column 1/.style={
    %   nodes={
    %     minimum width = 1em,
    %     text depth = 0em,
    %     fill=white,
    %     draw=white,
    %     text=
    %         black,
    %         font=\footnotesize,
    %         align=right,
    %   }
    % },
]

\tikzstyle{trace-table} = [
	table,
    row 1/.style={
      nodes={
        fill=white,
        draw=white,
        text=
            black,
            font=\footnotesize
      }
    }
]

\tikzstyle{eval-table} = [
    table,
]

\tikzstyle{link} = [
    arrows= {-Stealth},
    thick,
]

\noindent
\resizebox{\textwidth}{!}{
\newcommand{\cellw}{49ex}
\begin{tikzpicture}[
  node distance=0.8cm and 1.3cm,
  bend angle=45,
  font=\sffamily, 
  remember picture,
  auto,
]

\matrix[
  trace-table, 
  text width = \cellw,
] (l) {
 $i=0$ \& $i=1$ \& $i=2$ \\
\fuzzyval{0.5} \& \fuzzyval{0.9} \& \fuzzyval{0.2} \\
\fuzzyval{0.2} \& \fuzzyval{0.3} \& \fuzzyval{0.8} \\
};
\node[
    right=0mm of l-1-1.west,
    anchor=east,
] {$\lambda$};
\node[
    right=0mm of l-2-1.west,
    anchor=east,
] {$a$};
\node[
    right=0mm of l-3-1.west,
    anchor=east,
] {$b$};

\matrix[
  eval-table, 
  below= 0mm of l,
  text width = \cellw,
] (u) {
    %|[fill=\nucolorzero]|
    $
    \formulabox{f0}{v(\uformula,\lambda,0)}{Goldenrod} =
     \formulabox{b0}{v(b,\lambda,0)}{\atomcolor}
     \tor 
     (  \formulabox{a0}{v(a,\lambda,0)}{\atomcolor}
        \tand 
        \formulabox{u1}{v(\X(\uformula), \lambda, 0)}{Dandelion}
    )
    $
  \&
   $\formulabox{f1}{v(\uformula, \lambda, 1)}{Dandelion} =
   \formulabox{b1}{v(b,\lambda,1)}{\atomcolor}
     \tor 
     (  \formulabox{a1}{v(a,\lambda,1)}{\atomcolor}
        \tand 
        \formulabox{u2}{v(\X(\uformula), \lambda, 1)}{BurntOrange}
    )
   $
  \&
   $\formulabox{f2}{v(\uformula, \lambda, 2)}{BurntOrange} =
   \formulabox{b2}{v(b,\lambda,2)}{\atomcolor}
     \tor 
     (  \formulabox{a2}{v(a,\lambda,2)}{\atomcolor}
        \tand 
        \formulabox{u3}{v(\X(\uformula), \lambda, 2)}{\atomcolor}
    )
   $
  \\
  \fuzzyg{$\max\{$ 0.2 $,\min\{$ 0.5 $,$ 0.8 $\}\}=$ 0.5}{0.5}
  \&
  \fuzzyg{$ \max\{$ 0.3 $, \min\{$ 0.9 $,$ 0.8 $ \}\}=$ 0.8}{0.8}
  \&
  \fuzzyg{$\max\{$ 0.8 $,\min\{$ 0.2 $,$ 0 $\}\}=$ 0.8 $= v(b,\lambda,2)$}{0.8}
  \\
  \fuzzyp{0.2 + (0.5 $\cdot$ 0.8) - 0.2 $\cdot$ (0.5 $\cdot$ 0.8) $=$ 0.52}{0.52}
  \&
  \fuzzyp{0.3 + (0.9 $\cdot$ 0.8) - 0.3 $\cdot$ (0.9 $\cdot$ 0.8) $=$ 0.8}{0.8}
  \&
  \fuzzyp{0.8 + (0.2 $\cdot$ 0) - 0.8 $\cdot$ (0.2 $\cdot$ 0) $=$ 0.8 $= v(b,\lambda,2)$}{0.8}
  \\
  \fuzzyg{$\min\{$ 1$, $ 0.2 + $\max\{$ 0$, $ 0.5+1-1$\}\}=$ 0.7}{0.7}
  \&
  \fuzzyg{$\min\{$ 1$, $ 0.3 + $\max\{$ 0$, $ 0.9+0.8-1$\}\}=$ 1}{1}
  \&
  \fuzzyg{$\min\{$ 1$, $ 0.8 + $\max\{$ 0$, $ 0.2+0-1$\}\}=$ 0.8 $= v(b,\lambda,2)$}{0.8}
  \\
};
\node[
    right=0mm of u-1-1.west,
    anchor=east,
] {\uformula};
\node[
    right=0mm of u-2-1.west,
    anchor=east,
] {\textbf{G}};
\node[
    right=0mm of u-3-1.west,
    anchor=east,
] {\textbf{P}};
\node[
    right=0mm of u-4-1.west,
    anchor=east,
] {\textbf{L}};


\draw (a0.north) edge[link] (a0|-l-2-1.south);
\draw (b0.north) edge[link] (b0|-l-3-1.south);
\draw (a1.north) edge[link] (a1|-l-2-1.south);
\draw (b1.north) edge[link] (b1|-l-3-1.south);
\draw (a2.north) edge[link] (a2|-l-2-1.south);
\draw (b2.north) edge[link] (b2|-l-3-1.south);
\draw[out=30,in=150] (u1.north) edge[link] (f1.north);
\draw[out=30,in=150] (u2.north) edge[link] (f2.north);

% \matrix[
%   eval-table, 
%   below= 0mm of x2,
%   text width = \cellw,
% ] (x) {
%     |[fill=\nucolorzero]|
%     \formulabox{v(a \U b,\lambda,1)}{\ucolorone}
%   \&
%     |[fill=\nucolorone]|
%     \formulabox{v(a \U b,\lambda,2)}{\ucolortwo}
%   \&
%     |[fill=\nucolortwo]|
%     \formulabox{v(a \U b,\lambda,3)}{white}
%   \\
%   \fuzzyg{0}{0}
%   \&
%   \fuzzyg{0}{0}
%   \&
%   \fuzzyg{0}{0}
%   \\
%     \fuzzyp{0}{0}
%   \&
%   \fuzzyp{0}{0}
%   \&
%   \fuzzyp{0}{0}
%   \\
%   \fuzzyl{0}{0}
%   \&
%   \fuzzyl{0}{0}
%   \&
%   \fuzzyl{0}{0}
%   \\
% };
% \node[
%     right=0mm of x-1-1.west,
%     anchor=east,
% ] {\nuformula};
% \node[
%     right=0mm of x-2-1.west,
%     anchor=east,
% ] {\textbf{G}};
% \node[
%     right=0mm of x-3-1.west,
%     anchor=east,
% ] {\textbf{P}};
% \node[
%     right=0mm of x-4-1.west,
%     anchor=east,
% ] {\textbf{L}};


% \matrix[
%   eval-table, 
%   below= 0mm of x,
%   text width = \cellw,
% ] (a) {
%   |[text height=1.5em,fill=\acolorzero]|{$
%   \begin{aligned}
%     v(a,\lambda,0) 
%     \tor{}&
%     v(\X(a \U b),\lambda,0) \\
%     = 0.5 \tor{}& -
%     \end{aligned}$}
%   \&
%    |[text height=1.5em,fill=\acolorone]|{$
%     \begin{aligned}
%     \formulabox{v(a,\lambda,1)}{white} 
%     \tor{}&
%     \formulabox{v(\X(a \U b),\lambda,1)}{\ucolorone} \\
%     = 0.9 \tor{}& -
%     \end{aligned}$}
%    \&
%    |[text height=1.5em,fill=\acolortwo]|{$
%     \begin{aligned}
%     v(a,\lambda,2) 
%     \tor{}&
%     v(\X(a \U b),\lambda,2) \\
%     = 0.5 \tor{}& 0
%     \end{aligned}$}
%    \\
%   \fuzzyg{0}{0}
%   \&
%   \fuzzyg{0}{0}
%   \&
%   \fuzzyg{$\min(0.5,0) = 0$}{0}
%   \\
%    \fuzzyp{0}{0}
%   \&
%   \fuzzyp{0}{0}
%   \&
%   \fuzzyp{0}{0}
%   \\
%   \fuzzyl{0}{0}
%   \&
%   \fuzzyl{0}{0}
%   \&
%   \fuzzyl{$\min(1,0.5+0) = 0.5$}{0.5}
%   \\
% };
% \node[
%     right=0mm of a-1-1.west,
%     anchor=east,
% ] {$a \land \X(a \U b)$};
% \node[
%     right=0mm of a-2-1.west,
%     anchor=east,
% ] {\textbf{G}};
% \node[
%     right=0mm of a-3-1.west,
%     anchor=east,
% ] {\textbf{P}};
% \node[
%     right=0mm of a-4-1.west,
%     anchor=east,
% ] {\textbf{L}};

% \matrix[
%   eval-table, 
%   below= 0mm of a,
%   text width = \cellw,
% ] (u) {
%   |[text height=1.2em]|{$
%   \begin{aligned}
%     v(a,\lambda,0) 
%     \tor{}&
%     v(a \U b,\lambda,1) \\
%     = 0.5 \tor{}& -
%     \end{aligned}$}
%   \&
%    |[text height=1.2em]|{$
%     \begin{aligned}
%     v(a,\lambda,1) 
%     \tor{}&
%     v(a \U b,\lambda,2) \\
%     = 0.9 \tor{}& -
%     \end{aligned}$}
%    \&
%    |[text height=1.2em]|{$
%     \begin{aligned}
%     v(a,\lambda,2) 
%     \tor{}&
%     v(a \U b,\lambda,2) \\
%     = 0.5 \tor{}& 0
%     \end{aligned}$}
%    \\
%   \fuzzyg{0}{0}
%   \&
%   \fuzzyg{0}{0}
%   \&
%   \fuzzyg{$\min(0.5,0) = 0$}{0}
%   \\
%    \fuzzyp{0}{0}
%   \&
%   \fuzzyp{0}{0}
%   \&
%   \fuzzyp{0}{0}
%   \\
%   \fuzzyl{0}{0}
%   \&
%   \fuzzyl{0}{0}
%   \&
%   \fuzzyl{$\min(1,0.5+0) = 0.5$}{0.5}
%   \\
% };
% \node[
%     right=0mm of u-1-1.west,
%     anchor=east,
% ] {};%$a \U b = b \lor (a \land \X(a \U b))$};
% \node[
%     right=0mm of u-2-1.west,
%     anchor=east,
% ] {\textbf{G}};
% \node[
%     right=0mm of u-3-1.west,
%     anchor=east,
% ] {\textbf{P}};
% \node[
%     right=0mm of u-4-1.west,
%     anchor=east,
% ] {\textbf{L}};




\end{tikzpicture}
}




\begin{figure}
\centering
\resizebox{\linewidth}{!}{%

\begin{tikzpicture}[
    >=Stealth,
    every node/.style={font=\small},
    op/.style={draw,fill=white,minimum width=1.3cm,minimum height=0.6cm},
    %box/.style={draw,dashed,fill=green!15,inner sep=8pt},
    arr/.style={->,thick}
]

%----------------------------------------------------------
% Nodes inside the green box
%----------------------------------------------------------

\node[op] (minus) {$1-a$};

\node[right=3cm of minus] (veca)
{$\langle 0.2,0.9,0.8, *, *\rangle$};

\node[op,right=8cm of veca] (max)
{element-wise $\max$};

\node[right=3cm of max] (shiftvec)
{$\langle 0.7,0.7,0.7,*,*\rangle$};

\node[op,right=1.8cm of shiftvec] (shift)
{$\forall i, \oplus^{T-1}_i (\widetilde V_b)_{i,:}$};

%----------------------------------------------------------
% Bottom labels
%----------------------------------------------------------

\node[below=1.0cm of minus] (va)
{$\mathrm{V}_a=\langle0.8,0.1,0.2, * , *\rangle$};

\node[below=1.0cm of shift] (vb)
{$\mathrm{V}_b=\langle0.1,0.3,0.7,*,*\rangle$};

%----------------------------------------------------------
% Arrows inside
%----------------------------------------------------------

\draw[arr] (minus) -- (veca);
\draw[arr] (veca) -- (max);
\draw[arr] (shift) -- (shiftvec);
\draw[arr] (shiftvec) -- (max);

% Vertical arrows
\draw[arr] (va) -- (minus);

\draw[arr] (vb) -- (shift);

%----------------------------------------------------------
% Top computation
%----------------------------------------------------------

\node[above=0.2cm of max]
(vecab)
{$\neg a \lor \mathsf{F} b=\langle0.7,0.9,0.8,*,*\rangle$};

\node[above=0.1cm of shift]
(finally) {$\mathsf{F}b$};

\node[above=0.1cm of minus]
(neg) {$\neg a$} ;

\node[op,above=1cm of vecab] (min)
{$\min$};

\node[right=1.7cm of min]
(result)
{$v(G(a\rightarrow Fb),\lambda)=0.7$};

\draw[arr] (max) -- (min);
\draw[arr] (min) -- (result);

\end{tikzpicture}}
\caption{Graphical representation of Example~\ref{ex:trace_padding}}
\label{fig:placeholder}
\end{figure}

\todo{Paolo: 2 cose piccole, ma non voglio editare: farei le frecce da Va/Vb verso l'alto. Ed alla fine c'è Xb invece di Fb Andrei: Hai ragione, grazie.}



==> Sections/related.tex <==
\section{Related Work}
\label{sec:relatex}
%% Labels are used to cross-reference an item using \ref command.

This section discusses the related works from two main perspectives: neurosymbolic (NeSy) integration solutions applied for static, relational domains in Section~\ref{sec:static_nesy}, and NeSy solutions for temporal domains in Section~\ref{sec:temporal_nesy}. 
\subsection{Neurosymbolic Integration in static domains} 
\label{sec:static_nesy}
Neurosymbolic (NeSy) integration aims to bridge neural learning and structured reasoning. In static domains, the vast NeSy literature can be broadly classified based on where the symbolic knowledge is injected into the machine learning pipeline \cite{informed_ML}\footnote{In the broader taxonomy of informed machine learning \cite{informed_ML}, our ``loss-based'' and ``model-based'' categories correspond to integrating knowledge into the \emph{Learning Algorithm} and the \emph{Hypothesis Space}, respectively.}.

The first category comprises \emph{loss-based} approaches, where logic is strictly used to modify the learning algorithm (e.g., as a regularization term). In these frameworks, the neural network is penalized during training for violating logical constraints, but the symbolic component is discarded at inference time. The second category consists of \emph{model-based} approaches, which restrict the model's hypothesis space by embedding logic directly into the computational architecture, ensuring that logical reasoning persists during inference. The historical roots of this architectural integration can be traced back to KBANN \cite{KBANN}, which explicitly compiled symbolic rules into neural network topologies.

Orthogonally to this architectural divide, NeSy frameworks differ in the mathematical formalism used to evaluate logic. \emph{Probabilistic} approaches leverage probabilistic inference. Within this formalism, Semantic Loss \cite{DBLP:conf/icml/XuZFLB18} acts as a loss-based regularizer, whereas frameworks like DeepProbLog \cite{DBLP:conf/nips/ManhaeveDKDR18} and DeepStochLog \cite{DBLP:conf/aaai/WintersMMR22} act as model-based systems, piping neural outputs into probabilistic inference engines. However, the reliance on Weighted Model Counting (WMC) makes scaling probabilistic methods to complex formulas a significant computational bottleneck.

To overcome these scalability issues, \emph{fuzzy logic} frameworks leverage t-norms to translate discrete connectives into differentiable algebraic operations. %Applying the architectural distinction to this paradigm, 
Within the fuzzy logic paradigm, Logic Tensor Networks (LTN) \cite{ltn} and Semantic-Based Regularization (SBR) \cite{SBR} are popular loss-based fuzzy approaches. Conversely, model-based fuzzy approaches~\cite{KENN,DBLP:journals/ml/DanieleKSH23,Giunchiglia1, Giunchiglia2}, embed differentiable logical operations directly into the structure of neural networks through additional differentiable layers. Notably, these model-based methods are typically hardcoded to a specific t-norm semantics, which limits their flexibility across diverse domain constraints.

Despite the success of these frameworks in combining sub-symbolic and symbolic representations, a fundamental limitation shared by all these NeSy frameworks is the lack of native operators to model temporal dependencies.

In our work, we overcome these limitations by adopting a semantics-agnostic, model-based fuzzy paradigm for temporal data. By treating the formula as a differentiable computational layer, we enable scalable, instance-specific supervision that persists at inference time.
















% \todo[inline]{Bozza iniziale. TODO: aggiungere papers in più (per ora quelli già citati in \TILR), correggere un po' la scrittura, sistemare la parte finale di collegamento con la parte temporale. Forse si puo' togliere la distinzione tra model based e loss based qui, alla fine non è così rilevante.}

% Neurosymbolic (NeSy) integration aims to combine the robust learning capabilities of neural networks with the structured reasoning of symbolic logic. In static domains, this integration is broadly achieved through two main mathematical formalisms: exact probabilistic reasoning and fuzzy logic relaxations. 

% Probabilistic approaches, such as DeepProbLog \cite{DBLP:conf/nips/ManhaeveDKDR18}, DeepStochLog \cite{DBLP:conf/aaai/WintersMMR22}, and Semantic Loss \cite{DBLP:conf/icml/XuZFLB18}, define exact semantics over logic programs. In these frameworks, the outputs of neural perception modules are treated as probabilistic facts, allowing the system to perform structured logical inference. However, these methods typically rely on Weighted Model Counting (WMC) to compute the exact probability of a query. Since WMC is \#P-Complete, scaling probabilistic NeSy approaches to highly complex formulas remains a significant computational bottleneck.

% Alternatively, continuous or fuzzy logic frameworks leverage t-norms to translate discrete logical connectives into differentiable algebraic operations, scaling much better with formula complexity. Within this fuzzy paradigm, the architectural role of symbolic knowledge generally falls into two distinct categories: loss-based and model-based integration.\todo{In realtà, questa distinzione non è propria dei metodi basati su logica fuzzy, ma vale anche per metodi probabilistici}

% \todo[inline]{loss-based e model-based sono anche chiamati Learning Algorithm e Hypothesis Set, rispettivamente, in \cite{informed_ML} ("Informed Machine Learning – A Taxonomy and Survey of Integrating Prior Knowledge into Learning Systems"). Il paper è una literature review generale su integrazione di Prior Knolwegde (con knowledge espressa con logica come caso speciale). Contiene altre references utili.. Da citare e guardare per bene}

% In \emph{loss-based} approaches, such as Logic Tensor Networks (LTN) \cite{ltn} and Semantic-Based Regularization (SBR) \cite{SBR}, background knowledge is assumed to be strictly true. The logical formulas are translated directly into a loss function or a regularization term, penalizing the neural network during training whenever its predictions violate the given logical constraints. However, in these frameworks, the logical constraints are typically discarded after training and are not retained at inference time.

% Conversely, \emph{model-based} approaches integrate logic directly into the computational graph. Frameworks such as Knowledge Enhanced Neural Networks (KENN) \cite{KENN}, Iterative Local Refinement (ILR) \cite{DBLP:journals/ml/DanieleKSH23}, and other differentiable fuzzy layers \cite{Giunchiglia1, Giunchiglia2} embed logical operations as differentiable components downstream of the neural feature extractors. In this setting, the logic computes a dynamic degree of satisfaction based on the latent neural perceptions. This aggregated logical output is then supervised against instance-specific target values using standard loss functions (e.g., Binary Cross-Entropy). 

% Crucially, this model-based integration of fuzzy logic is the exact architectural paradigm we adopt in our work. By treating the formula as a differentiable computational layer rather than a global prior, we enable instance-specific supervision that persists at inference time.

% Despite their success in bridging the sub-symbolic and symbolic divide, a fundamental limitation shared by all the aforementioned NeSy frameworks is the lack of native operators to model chronological dependencies. Applying propositional or first-order logic to temporal tasks requires manual aggregation of sequences or spatial unrolling of time, which fails to capture the explicit dynamics of the domain. This limitation motivates the extension of differentiable logic paradigms to explicit temporal reasoning.


\subsection{Neurosymbolic Integration in dynamic domains}
\label{sec:temporal_nesy}
% umili fuzzy dfa 
% -> visual reward machines, suffix predicton
% DeepDFA ? dfa induction
% nesy A
% dire, come nel paper nesy, "rely on DFA construction, which poses computational
% challenges due to the costly ltlf to DFA conversion (De Giacomo and Vardi, 2013)."
% per collegarsi a
% valutazione diretta senza dfa: \TILR

% The most diffused approaches for integrating \LTLF specifications into neural architectures relies on an intermediate automaton representation.
% The \LTLF formula is first compiled into a deterministic finite-state automaton (DFA), which is then interpreted differentiably over the neural network's outputs.
Existing temporal NeSy approaches largely rely on the compilation of the \LTLF specification into a finite-state automaton, which is then interpreted differentiably over the neural perception outputs.
\FuzzyDFA \cite{DBLP:conf/kr/UmiliCG23} adopts a fuzzy interpretation, and has been adapted to non-Markovian reinforcement learning \cite{DBLP:conf/nesy/UmiliABC23} and to suffix prediction under \LTLF constraints \cite{DBLP:conf/pmai/UmiliLP24}.
\NeSyA \cite{DBLP:conf/ijcai/ManginasPR25} adopts a probabilistic interpretation. 
Section~\ref{sec:temporal_nesy} covers the functioning principles of both. 
% Umili et al. \cite{DBLP:conf/kr/UmiliCG23} introduced this framework for weakly supervised sequence classification: the \LTLF formula is translated into a DFA, and each transition guard is evaluated as a fuzzy propositional formula over the output of a neural perception module. State distributions are propagated recursively over the sequence.
% The same DFA-based mechanism has been extended to non-Markovian reinforcement learning \cite{DBLP:conf/nesy/UmiliABC23} and to suffix prediction under \LTLF constraints \cite{DBLP:conf/pmai/UmiliLP24}.
% % DeepDFA ?
% 
% \NeSyA \cite{DBLP:conf/ijcai/ManginasPR25} replaces the fuzzy semantics with exact probabilistic reasoning. The \LTLF formula is compiled into a symbolic finite-state automaton (SFA), whose transition guards are compiled into d-DNNF circuits for weighted model counting (WMC). At each timestep, the WMC of each guard yields a transition probability, and the state distribution is updated via matrix multiplication.
% Both \FuzzyDFA and \NeSyA share a dependence on the explicit construction of a finite-state automaton, whose number of states can be double-exponential in the size of the \LTLF formula \cite{DBLP:conf/ijcai/GiacomoV13}. % frase presa e modificata da paper \FuzzyDFA
The \LTLZinc benchmark \cite{ltlzincIJCAI} evaluates these DFA-based methods within a modular pipeline for sequence classification with relational and temporal knowledge constraints across a series of different tasks, where however additional supervision signals are required in order to ensure that the compared methods are able to learn the prediction tasks. 

A separate line of work evaluates temporal specification directly through fuzzy semantics, without compiling an automaton. \citet{DonadelloFIMM25} use this approach for conformance checking of fuzzy event logs under Gödel semantics. \TILR \cite{DBLP:conf/nesy/AndreoniBDGMR25} introduced a first neurosymbolic instantiation for weakly supervised learning, based on iterative local refinement.

\todo[inline]{CHIARA: scritti cosi' i related potrebbero stare all'inizio. Se li mettimao alla fine mi aspetterei una comparison ESPLICITA tra i metodi temporali esistenti e \DiffLTLf, che secondo me e' da aggiungere. E' anche strano che i related con i lavori temporali sono piu' corti di quelli statici.}

==> Sections/results_old.tex <==
                \section{Results}
\label{sec:results}
%% Labels are used to cross-reference an item using \ref command.

% Struttura:
% - preambolo (poche frasi) per richiamare le RQs, dire che i risultati sono la media di 10 runs, il test statistico usato, e gli hyperparams
% - parte 1 (impatto della semantica fuzzy) RQ1
%     - confronto di goedel, prod, luk, sugli esperimenti formula-complessità
%     - risultato: product è la più consistent. le altre ottengono ottimi risultati con 2 classi ma degradano con l'aumentare della complessità della formula e hanno molta varianza (minimi locali). product è stabile
%     - conclusione: selezioniamo product come semantica rappresentativa per RQ2 e RQ3
% - parte 2 (confronto con lo stato dell'arte) RQ2-3
%     - mostriamo che \DiffLTLf (product) ha pari o superiore acc dei competitors
%     - mostriamo che è molto più veloce
% - limiti:
%     - benchmark sintetico
%     - dimensione del dataset (ma giustificabile dicendo che i metodi dfa-based hanno il limite di non poter trattare dataset troppo vasti, per problemi di scalabilità)
%     - abbiamo testato solo un tipo di perception (CNN). In realtà non è un grosso limite dato che stiamo confrontando il modulo logico

This section presents the experimental results structured around three research questions.
\textbf{RQ1} (Section \ref{sec:results_rq1}) investigates the impact of the fuzzy semantics on the symbol grounding accuracy performance within \DiffLTLf. Next,
\textbf{RQ2} (Section \ref{sec:results_rq2}) compares the best-performing \DiffLTLf semantic configuration against state-of-the-art temporal neurosymbolic methods in term of classification accuracy at both the sequence and symbol grounding level.
\textbf{RQ3} (Section \ref{sec:results_rq3}) evaluates the computational scalability of the compared methods.
All results are averaged over 10 independent runs. As all methods share seeds, splits, and sampled sequences, differing only in the logic module, statistical significance is assessed 
with a paired one-sided Wilcoxon signed-rank test. Throughout, results marked in bold denote a method that is significantly better than all
competitors at $p<0.05$.


\subsection{Impact of Fuzzy Temporal Semantics}
\label{sec:results_rq1}

\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{Figures/fuzzy_semantics_comparison.pdf}
  \caption{Symbol grounding accuracy (\%) across 
  10 independent runs for \DiffLTLf instantiated with the three fuzzy semantics: Gödel 
  (\FLTLF[G]), Product (\FLTLF[P]), and Łukasiewicz (\FLTLF[L]). 
  Each subplot corresponds to one experimental setting (formula 
  set $\times$ image dataset), with the number of classes $|\mathcal{C}|$ on the horizontal axis.}
  \label{fig:acc_semantics}
\end{figure}

We first evaluate the effect of the underlying fuzzy semantics on classification performance. 
Specifically, we compare the three instantiations of \FLTLF introduced in Section \ref{sec:fuzzyLTL}: Gödel (\FLTLF[G]), Product (\FLTLF[P]), and Łukasiewicz (\FLTLF[L]). 
% The comparison is conducted on the formula-complexity benchmark described in Section \ref{sec:evaluation_formula}, 
% across all four experimental settings (formulas set 1 and 2, on both MNIST and Fashion-MNIST datasets), with the number of conjuncted sub-formulas ranging from $K=1$ to $K=4$, and correspondingly the number of classes $|\mathcal{C}| = 2K$ ranging from $2$ to $8$.
The comparison is conducted across all four experimental settings of Section~\ref{sec:formula_complexity}, with the number of classes ranging from $|\mathcal{C}|=2$ to $|\mathcal{C}|=8$.

Figure \ref{fig:acc_semantics} shows the results on the symbol grounding accuracy across runs for each semantics and each value of $|\mathcal{C}|$. At $|\mathcal{C}|=2$, where the temporal specification involves only two classes, all three semantics achieve comparable performances, with median grounding accuracy above $99\%$ in almost all settings. Differences emerge as the formula complexity increases, as both Gödel and Łukasiewicz exhibit a significant increase in variance. For $|\mathcal{C}|=4$, while these two semantics occasionally reach near optimal level of performance, many runs converge to lower values. For $|\mathcal{C}|\geq 6$, the degradation of performance becomes more severe.
This pattern suggests sensitivity to local optima during training, which we cover below.
In contrast, Product semantics maintains consistently high grounding accuracy with low variance across all values of $|\mathcal{C}|$ and across all settings.

This pattern is consistent with prior findings in non-temporal neurosymbolic settings, where Product logic has been shown to provide more informative gradients than Gödel and Łukasiewicz for constraint satisfaction tasks \cite{DBLP:journals/ai/KriekenAH22}. The present results extend this observation to the temporal domain and can be explained by analysing the gradient properties of the underlying operators. 
In our setting, the temporal operators $\always$ and $\eventually$ reduce to iterated applications of the t-norm and t-conorm respectively, over the trace length.

Under \textbf{Product semantics}, the t-norm $\alpha \tand \beta = \alpha \cdot \beta$ has partial derivative $\beta$ with respect to $\alpha$, and the t-conorm $\alpha \oplus \beta = \alpha + \beta - \alpha \cdot \beta$ has partial derivative $1 - \beta$.
Both are non-vanishing on almost the entire input domain. As a result, when $\always$ is evaluated over a trace of length $n$, 
% every input at each timestep 
every timestep receives a non-zero gradient, enabling the perception module to update all its predictions in each training step.

Under \textbf{Gödel semantics}, the $\min$ and $\max$ operators are single-passing. At most one of their arguments receives a non-zero gradient.
As shown in~\cite{DBLP:journals/ai/KriekenAH22}, any composition of single-passing functions is itself single-passing. 
As a consequence, the entire computation graph derived from a temporal formula inherits this property.
Concretely, given a sequence of $n$ observations, at most one receives a non-zero gradient. For this reason, convergence becomes sensitive to which single observation happens to receive the learning signal.
This makes learning increasingly hard as $|\mathcal{C}|$ grows, explaining the performance degradation and high variance observed in Figure~\ref{fig:acc_semantics}.

Under \textbf{Łukasiewicz semantics}, the t-norm $\alpha \otimes \beta = \max(\alpha + \beta - 1, 0)$ has gradient $1$ when $\alpha + \beta > 1$ and $0$ otherwise.
For the $n$-ary case, which corresponds to the evaluation of $\always$ over a trace of length $n$, van Krieken et al.~\cite{DBLP:journals/ai/KriekenAH22} show that the gradient is non-vanishing only when the mean truth value of the $n$ arguments is greater than $(n-1)/n$, and that the fraction of the input space satisfying this condition is $1/n!$. 
This condition is particularly difficult to verify, especially during early training, when the perception module produces output with intermediate truth values.
The t-conorm $\min(\alpha + \beta, 1)$, shows a symmetrical issue, with its gradient vanishing when the sum of its arguments exceeds $1$. 
As $|\mathcal{C}|$ increases, the outer conjunction further stresses the problem. This explains the performance degradation at higher $|\mathcal{C}|$ (Figure~\ref{fig:acc_semantics}).

Based on these findings, all subsequent experiments adopt \FLTLF[P] Product semantics as the default configuration of \DiffLTLf.

\subsection{Comparison with State of the Art}
\label{sec:results_rq2}
\begin{table*}[ht]
\centering
\caption{Performance comparison varying formula complexity. Results are averaged over 10 independent runs.
\textbf{Img. Acc}: Symbol Grounding Accuracy; 
\textbf{Seq. Acc}: Sequence Classification Accuracy; 
\textbf{Time}: Logic Module Time per Epoch. 
Results in \textbf{bold} are statistically significantly better than all other methods (Wilcoxon, $p<0.05$).}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc ccc ccc ccc}
\toprule
& & \multicolumn{3}{c}{\textbf{Img. Acc.} ($\%$) $\uparrow$} & \multicolumn{3}{c}{\textbf{Seq. Acc.} ($\%$) $\uparrow$} & \multicolumn{3}{c}{\textbf{Time} (s) $\downarrow$} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Setting & $|\mathcal{C}|$ & \DiffLTLf & \FuzzyDFA & \NeSyA & \DiffLTLf & \FuzzyDFA & \NeSyA & \DiffLTLf & \FuzzyDFA & \NeSyA \\
\midrule
\multirow{4}{*}{\shortstack[l]{MNIST\\Set1}} & 2 & 99.9 & 99.9 & 99.9 & 99.8 & 99.8 & 99.8 & \textbf{0.04} & 0.17 & 0.17 \\
 & 4 & 97.4 & 97.4 & 97.4 & 98.9 & 98.9 & 99.0 & \textbf{0.05} & 0.33 & 0.40 \\
 & 6 & 95.7 & 95.6 & 91.3 & 98.3 & 98.3 & 97.6 & \textbf{0.05} & 0.63 & 0.99 \\
 & 8 & 92.7 & 91.5 & 88.4 & 96.7 & 96.5 & 95.5 & \textbf{0.05} & 1.97 & 5.08 \\
\midrule
\multirow{4}{*}{\shortstack[l]{MNIST\\Set2}} & 2 & 99.9 & 99.9 & 99.9 & 99.8 & 99.9 & 99.9 & \textbf{0.05} & 0.17 & 0.15 \\
 & 4 & 97.4 & 97.3 & 97.3 & 99.0 & 99.1 & 99.0 & \textbf{0.06} & 0.34 & 0.37 \\
 & 6 & 95.0 & 95.0 & 95.0 & 98.1 & 98.2 & 98.1 & \textbf{0.06} & 0.69 & 0.88 \\
 & 8 & 92.7 & 92.7 & 92.7 & 98.0 & 98.0 & 97.9 & \textbf{0.07} & 4.86 & 10.38 \\
\midrule
\multirow{4}{*}{\shortstack[l]{F-MNIST\\Set1}} & 2 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & \textbf{0.04} & 0.14 & 0.30 \\
 & 4 & 97.8 & 97.9 & 97.9 & 98.7 & 98.7 & \textbf{98.8} & \textbf{0.05} & 0.35 & 0.59 \\
 & 6 & 91.7 & 91.7 & \textbf{92.0} & 95.5 & 95.3 & 95.7 & \textbf{0.05} & 0.69 & 1.27 \\
 & 8 & 86.0 & 85.6 & 83.9 & 93.2 & 93.2 & 92.8 & \textbf{0.05} & 2.24 & 5.42 \\
\midrule
\multirow{4}{*}{\shortstack[l]{F-MNIST\\Set2}} & 2 & 99.9 & 99.9 & 99.9 & 99.9 & 99.9 & 99.9 & \textbf{0.05} & 0.14 & 0.14 \\
 & 4 & 98.0 & 98.0 & 98.0 & 99.0 & 98.9 & 99.0 & \textbf{0.05} & 0.25 & 0.34 \\
 & 6 & 90.9 & 91.1 & 91.0 & 96.2 & 96.3 & 96.1 & \textbf{0.06} & 0.71 & 0.87 \\
 & 8 & 85.1 & 85.6 & 85.4 & 96.2 & 96.2 & 96.4 & \textbf{0.07} & 4.83 & 10.49 \\
\bottomrule
\end{tabular}}
\label{tab:formula_complexity}
\end{table*}








Having established the superior performance of the Product semantics, we now compare \DiffLTLf under Product semantics against two state-of-the-art temporal neurosymbolic methods: \FuzzyDFA\footnote{We use the \FuzzyDFA implementation from the \LTLZinc benchmark \cite{ltlzincIJCAI}, which deviates from the original in state normalisation and training loss; see \ref{app1} for a precise description.} \cite{DBLP:conf/kr/UmiliCG23} and \NeSyA \cite{DBLP:conf/ijcai/ManginasPR25}.
The comparison is conducted along two complementary directions: increasing the formula complexity (Table~\ref{tab:formula_complexity}) and increasing the sequence length (Table~\ref{tab:seq_length}).
Both tables also report the logic module time per epoch. Computational scalability is discussed separately in Section \ref{sec:results_rq3}.
Additionally, we include two purely neural baselines (where the logic module is replaced by a GRU \cite{DBLP:conf/emnlp/ChoMGBBSB14} and a Transformer encoder \cite{DBLP:conf/nips/VaswaniSPUJGKP17}, respectively) in the visual comparison. Their complete numerical results are reported in \ref{app:full_results}.

\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{Figures/formula_complexity_comparison.pdf}
  \caption{Comparison of symbol grounding accuracy (left) and logic module time per epoch (right) across number of classes $|\mathcal{C}| \in \{2,4,6,8\}$. Values are averaged across all four experimental settings (formula set $\times$ image dataset).}
  
  \label{fig:formula_complexity}
\end{figure}

\paragraph{Varying formula complexity} 
Table~\ref{tab:formula_complexity} and Figure~\ref{fig:formula_complexity} report classification performance as the number of classes $|\mathcal{C}|$ increases from $2$ to $8$. 
At $|\mathcal{C}|=2$, all three neurosymbolic methods achieve near-perfect grounding accuracy across all settings, with almost no statistically significant differences. As the symbolic complexity grows, the three methods remain competitive with no single method consistently superior across all configurations.
% The two neural baselines confirm the necessity of explicit temporal logic rule injection, as they prove to be inadequate for this weakly-supervised learning task.
The two purely neural baselines fail to learn a valid symbol grounding, 
as their grounding accuracy collapsed towards chance level as $|\mathcal{C}|$ grows (Figure~\ref{fig:formula_complexity}, left), confirming that explicit temporal logic injection is necessary for this weakly-supervised task.


% \begin{table*}[ht]
% \centering
% \caption{Performance comparison varying sequence length. Results are averaged over 10 independent runs.
% \textbf{Img. Acc}: Symbol Grounding Accuracy; 
% \textbf{Seq. Acc}: Sequence Classification Accuracy; 
% \textbf{Time}: Logic Module Time per Epoch. 
% Results in \textbf{bold} are statistically significantly better than all other methods.}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c ccc ccc ccc}
% \toprule
% & \multicolumn{3}{c}{\textbf{Img. Acc.} ($\% \uparrow$)} & \multicolumn{3}{c}{\textbf{Seq. Acc.} ($\% \uparrow$)} & \multicolumn{3}{c}{\textbf{Time} (s $\downarrow$)} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% Len & \DiffLTLf & \FuzzyDFA & \NeSyA & \DiffLTLf & \FuzzyDFA & \NeSyA & \DiffLTLf & \FuzzyDFA & \NeSyA \\
% \midrule
% 20 & 95.8 & 95.3 & 95.8 & 95.3 & 94.0 & 95.5 & \textbf{0.16} & 2.32 & 3.43 \\
% 40 & 96.0 & 95.6 & 96.0 & 94.5 & 92.8 & 94.7 & \textbf{0.30} & 4.73 & 6.90 \\
% 60 & \textbf{95.6} & 94.7 & 95.4 & \textbf{94.7} & 92.2 & 94.1 & \textbf{0.44} & 7.12 & 10.45 \\
% 80 & \textbf{95.7} & 94.6 & 95.4 & 95.0 & 93.5 & 94.2 & \textbf{0.62} & 9.56 & 13.93 \\
% 100 & 95.6 & 94.2 & 95.6 & 94.5 & 90.1 & 94.2 & \textbf{0.79} & 11.91 & 17.39 \\
% 120 & \textbf{95.5} & 93.6 & 94.7 & \textbf{93.0} & 90.0 & 91.8 & \textbf{0.95} & 14.35 & 21.00 \\
% 140 & \textbf{96.1} & 93.7 & 95.5 & \textbf{93.5} & 88.9 & 91.8 & \textbf{1.11} & 16.72 & 24.64 \\
% 160 & \textbf{95.8} & 94.2 & 95.3 & 94.0 & 90.5 & 92.9 & \textbf{1.25} & 19.09 & 27.87 \\
% 180 & \textbf{95.8} & 88.3 & 95.3 & \textbf{93.7} & 83.2 & 91.8 & \textbf{1.42} & 21.58 & 29.88 \\
% 200 & \textbf{95.6} & 92.2 & 95.0 & \textbf{94.7} & 86.3 & 92.9 & \textbf{1.57} & 23.84 & 32.58 \\
% \bottomrule
% \end{tabular}}
% \label{tab:scalability_results}
% \end{table*}


% \begin{table*}[ht]
% \centering
% \caption{\riccardo{Esperimenti su formula "(G(x0 -> F(y1))) \& (G(y2 -> F(z3)))"}}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c ccc ccc ccc}
% \toprule
% & \multicolumn{3}{c}{\textbf{Img. Acc.} ($\% \uparrow$)} & \multicolumn{3}{c}{\textbf{Seq. Acc.} ($\% \uparrow$)} & \multicolumn{3}{c}{\textbf{Time} (s $\downarrow$)} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% Len & \DiffLTLf & \FuzzyDFA & \NeSyA & \DiffLTLf & \FuzzyDFA & \NeSyA & \DiffLTLf & \FuzzyDFA & \NeSyA \\
% \midrule
% 20 & 97.9 & 97.9 & \textbf{98.0} & 97.7 & 97.8 & 97.8 & \textbf{6.53e-03} & 0.41 & 0.57 \\
% 40 & 97.9 & 98.0 & 98.0 & 98.0 & 98.1 & 98.1 & \textbf{6.66e-03} & 0.74 & 1.14 \\
% 60 & 97.9 & 98.1 & \textbf{98.1} & 97.2 & 97.7 & 97.6 & \textbf{6.71e-03} & 1.09 & 1.74 \\
% 80 & 98.0 & 97.9 & 97.9 & 98.0 & 98.2 & 98.2 & \textbf{6.92e-03} & 1.46 & 2.33 \\
% 100 & 98.0 & 98.0 & \textbf{98.1} & 98.1 & 98.0 & 98.0 & \textbf{7.84e-03} & 1.83 & 2.91 \\
% 120 & 97.9 & 97.9 & 97.9 & 98.0 & 98.2 & 98.0 & \textbf{8.06e-03} & 2.21 & 3.53 \\
% 140 & 98.1 & 98.1 & 98.1 & 98.9 & 99.0 & 99.0 & \textbf{7.95e-03} & 2.59 & 4.12 \\
% 160 & 97.7 & 97.7 & \textbf{97.8} & 97.3 & 97.2 & 97.3 & \textbf{8.17e-03} & 2.96 & 4.74 \\
% 180 & 97.9 & 98.0 & \textbf{98.0} & 98.4 & 98.5 & 98.5 & \textbf{8.24e-03} & 3.31 & 5.34 \\
% 200 & 97.7 & 97.8 & 97.8 & 97.6 & 97.5 & 97.6 & \textbf{8.06e-03} & 3.69 & 5.89 \\
% \bottomrule
% \end{tabular}}
% \label{tab:scalability_results}
% \end{table*}

\begin{table*}[ht]
\centering
\caption{Performance comparison varying sequence length. 
Results are averaged over 10 independent runs.
\textbf{Img. Acc}: Symbol Grounding Accuracy; 
\textbf{Seq. Acc}: Sequence Classification Accuracy; 
\textbf{Time}: Logic Module Time per Epoch. 
Results in \textbf{bold} are statistically significantly 
better than all other methods (Wilcoxon, $p<0.05$).}
\resizebox{\textwidth}{!}{
\begin{tabular}{cc ccc ccc ccc}
\toprule
& & \multicolumn{3}{c}{\textbf{Img. Acc.} ($\%$) $\uparrow$} 
& \multicolumn{3}{c}{\textbf{Seq. Acc.} ($\%$) $\uparrow$} 
& \multicolumn{3}{c}{\textbf{Time} (s) $\downarrow$} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
$|\mathcal{C}|$ & Len & \DiffLTLf & \FuzzyDFA & \NeSyA 
& \DiffLTLf & \FuzzyDFA & \NeSyA 
& \DiffLTLf & \FuzzyDFA & \NeSyA \\
\midrule
\multirow{10}{*}{4}
 & 20  & 97.9 & 97.9 & \textbf{98.0} & 97.7 & 97.8 & 97.8 & \textbf{0.007} & 0.41 & 0.57 \\
 & 40  & 97.9 & 98.0 & 98.0 & 98.0 & 98.1 & 98.1 & \textbf{0.007} & 0.74 & 1.14 \\
 & 60  & 97.9 & 98.1 & \textbf{98.1} & 97.2 & 97.7 & 97.6 & \textbf{0.007} & 1.09 & 1.74 \\
 & 80  & 98.0 & 97.9 & 97.9 & 98.0 & 98.2 & 98.2 & \textbf{0.007} & 1.46 & 2.33 \\
 & 100 & 98.0 & 98.0 & \textbf{98.1} & 98.1 & 98.0 & 98.0 & \textbf{0.008} & 1.83 & 2.91 \\
 & 120 & 97.9 & 97.9 & 97.9 & 98.0 & 98.2 & 98.0 & \textbf{0.008} & 2.21 & 3.53 \\
 & 140 & 98.1 & 98.1 & 98.1 & 98.9 & 99.0 & 99.0 & \textbf{0.008} & 2.59 & 4.12 \\
 & 160 & 97.7 & 97.7 & \textbf{97.8} & 97.3 & 97.2 & 97.3 & \textbf{0.008} & 2.96 & 4.74 \\
 & 180 & 97.9 & 98.0 & \textbf{98.0} & 98.4 & 98.5 & 98.5 & \textbf{0.008} & 3.31 & 5.34 \\
 & 200 & 97.7 & 97.8 & 97.8 & 97.6 & 97.5 & 97.6 & \textbf{0.008} & 3.69 & 5.89 \\
\midrule
\multirow{10}{*}{8}
 & 20  & 95.8 & 95.3 & 95.8 & 95.3 & 94.0 & 95.5 & \textbf{0.16} & 2.32 & 3.43 \\
 & 40  & 96.0 & 95.6 & 96.0 & 94.5 & 92.8 & 94.7 & \textbf{0.30} & 4.73 & 6.90 \\
 & 60  & \textbf{95.6} & 94.7 & 95.4 & \textbf{94.7} & 92.2 & 94.1 & \textbf{0.44} & 7.12 & 10.45 \\
 & 80  & \textbf{95.7} & 94.6 & 95.4 & 95.0 & 93.5 & 94.2 & \textbf{0.62} & 9.56 & 13.93 \\
 & 100 & 95.6 & 94.2 & 95.6 & 94.5 & 90.1 & 94.2 & \textbf{0.79} & 11.91 & 17.39 \\
 & 120 & \textbf{95.5} & 93.6 & 94.7 & \textbf{93.0} & 90.0 & 91.8 & \textbf{0.95} & 14.35 & 21.00 \\
 & 140 & \textbf{96.1} & 93.7 & 95.5 & \textbf{93.5} & 88.9 & 91.8 & \textbf{1.11} & 16.72 & 24.64 \\
 & 160 & \textbf{95.8} & 94.2 & 95.3 & 94.0 & 90.5 & 92.9 & \textbf{1.25} & 19.09 & 27.87 \\
 & 180 & \textbf{95.8} & 88.3 & 95.3 & \textbf{93.7} & 83.2 & 91.8 & \textbf{1.42} & 21.58 & 29.88 \\
 & 200 & \textbf{95.6} & 92.2 & 95.0 & \textbf{94.7} & 86.3 & 92.9 & \textbf{1.57} & 23.84 & 32.58 \\
\bottomrule
\end{tabular}}
\label{tab:seq_length}
\end{table*}


\begin{figure}[t]
  \centering
  \includegraphics[width=\textwidth]{Figures/seq_length_comparison_combined.pdf}
  \caption{Comparison of symbol grounding accuracy (top row) and logic module time per epoch (bottom row) across sequence lengths varying from 20 to 200.
  Left column: temporal specification with $|\mathcal{C}|=4$ classes. 
  Right column: temporal specification with $|\mathcal{C}|=8$ classes.
  Lines represent the mean over 10 independent runs; shaded bands indicate the range between the minimum and maximum values.
  Time is shown on a logarithmic scale.}
  
  \label{fig:sequence_len}
\end{figure}
\paragraph{Varying sequence length} 
Table~\ref{tab:seq_length} and Figure~\ref{fig:sequence_len} report the performance as the sequence length increases from 20 to 200, following the setup described in Section~\ref{sec:varying_length}.
% Unlike the previous setting, here all sequences within each configuration share the same fixed length, so as to isolate the effect of sequence length on learning performance.
% The temporal specification is ... \todo{qui spendere 2 frasi per spiegare la scelta della formula logica e le motivazioni (distribuzione classi costante al variare di L)} ... involving 8 classes.

With $|\mathcal{C}|=4$, all three methods achieve high and stable grounding accuracy across the entire range of sequence lengths. \NeSyA achieves statistically significant improvements over both competitors at several lengths; however, the absolute differences are negligible. In practice, the three methods are indistingushable in terms of accuracy on this specification.

Differently, with $|\mathcal{C}|=8$, at short sequence lengths \DiffLTLf and \NeSyA achieve comparable grounding accuracy. However, as the sequence length increases, both \FuzzyDFA and \NeSyA show performance degradation and fall behind \DiffLTLf in both image and sequence classification accuracy, with statistically significant differences appearing from length 60 onward. Such degradation is not visible in for \DiffLTLf, which maintains stable grounding accuracy across the entire range of sequence lengths. 

% At short sequence lengths, \DiffLTLf and \NeSyA achieve comparable grounding accuracy. As the sequence length increases, both \FuzzyDFA and \NeSyA show performance degradation and fall behind \DiffLTLf in both image and sequence classification accuracy, with statistically significant differences appearing from length 60 onward. Such degradation is not visible in for \DiffLTLf, which maintains stable grounding accuracy across the entire range of sequence lengths.

For clarity, the two purely neural baselines are omitted from
Figure~\ref{fig:sequence_len} and Table~\ref{tab:seq_length}, as they do not reach a valid solution on this task (grounding accuracy close to chance across all sequence lengths).
Their complete numerical results are reported in~\ref{app:full_results}.

\paragraph{Summary} 
In the formula-complexity setting, no method consistently outperforms the others: the three neurosymbolic approaches achieve comparable accuracy across all tested configurations. In the sequence-length setting, when the temporal specification is simple ($|\mathcal{C}|=4$), all methods perform comparably. When the specification complexity increases ($|\mathcal{C}|=8$), \DiffLTLf shows an advantage over the DFA-based methods, maintaining stable performances as the problem difficulty increases, while both competitors' performances degrade.
The following section shows that this accuracy is achieved at a fraction of the computational cost.


\subsection{Computational Scalability}
\label{sec:results_rq3}
\todo[inline]{Andrei: qui secondo me possono andare le considerazione che avevo in temporal nesy su perche' \NeSyA va cosi lento e fuzzy dfa un po' meglio, e }
We now focus on the computational cost of the compared methods, measured as the logic module time per training epoch. This metric isolates the overhead introduced by the temporal symbolic reasoning component, as the perception module is identical across all methods.

The time columns of Tables~\ref{tab:formula_complexity} and~\ref{tab:seq_length} highlight a consistent and significant gap between \DiffLTLf and both DFA-based methods. In the formula-complexity setting, the time required by \DiffLTLf is essentially invariant with respect to $K$: increasing the number of sub-formulas from 1 to 4 produces negligible overhead (from 0.04\,s to 0.07\,s per epoch).
This is expected, since \DiffLTLf evaluates the formula compositionally on the trace and does not require the construction of an automaton whose state space may grow exponentially with the formula structure. In contrast, both \FuzzyDFA and \NeSyA rely on DFA-based representations, whose size and associated differentiable computations increase with the complexity of the specification; as a result, their training time grows significantly with $K$, with \NeSyA exceeding 10\,s per epoch at $|\mathcal{C}|=8$.
%\todo[inline]{Andrei: Darei una spiegazione, per la tabella 3 per le differenze del tempo tra c = 4 e c = 8 per \DiffLTLf. Penso sia la proposizzionalizazione e la complessita della formula che fanno aumentare il tempo. Cosi' si' puo' attacare anche la spiegazione dell'esplozione dell DFA.}
The two purely neural baselines attain even lower per-epoch times, as they avoid any symbolic computation. Their speed, however, is not meaningful in this setting since they do not learn the task (near-chance grounding accuracy).

In the sequence-length setting (Table~\ref{tab:seq_length}), all three neurosymbolic methods scale linearly with sequence length, as expected. However, at any given length, DFA-based require over an order of magnitude more time than \DiffLTLf. This holds for both 
tested specifications, and confirms the efficiency of \DiffLTLf to integrate the temporal specifications within the training procedure. 
It is worth noting that the reported times only account for training and do not include the cost of constructing the DFA. 

Combined with the accuracy result of Section \ref{sec:results_rq2}, these results prove that direct fuzzy evaluation of specifications \LTLF achieves comparable or higher classification accuracy than DFA-based methods while requiring a fraction of the computational cost. 
%\todo{dire che non consideriamo il costo di costruzione del DFA}



